21 cm Line Astronomy and Constraining New Physics

The 21 cm signal appears to be a treasure trove to provide an insight into the period when the first generation of luminous objects formed in the Universe. Hydrogen is the predominating fraction of the total baryonic matter during cosmic dawn (CD). Therefore, it is convenient and advantageous to study physics during CD using the 21 cm signal. The presence of any exotic source of energy can inject energy into the intergalactic medium (IGM) and heat the gas. Subsequently, it can modify the absorption amplitude in the global 21 cm signal. This feature can provide a robust bound on such sources of energy injection into the IGM gas.

==> chapter7.tex <==



